Loss Gradient Gaussian Width based Generalization and Optimization Guarantees

Generalization and optimization guarantees on the population loss often rely on uniform convergence based analysis, typically based on the Rademacher complexity of the predictors. The rich representation power of modern models has led to concerns about this approach. In this paper, we present generalization and optimization guarantees in terms of the complexity of the gradients, as measured by the Loss Gradient Gaussian Width (LGGW). First, we introduce generalization guarantees directly in terms of the LGGW under a flexible gradient domination condition, which includes the popular PL (Polyak-{\L}ojasiewicz) condition as a special case. Second, we show that sample reuse in iterative gradient descent does not make the empirical gradients deviate from the population gradients as long as the LGGW is small. Third, focusing on deep networks, we bound their single-sample LGGW in terms of the Gaussian width of the featurizer, i.e., the output of the last-but-one layer. To our knowledge, our generalization and optimization guarantees in terms of LGGW are the first results of its kind, and hold considerable promise towards quantitatively tight bounds for deep models.

==> arXiv_v3/sections/gauss_width_arxiv.tex <==

%\yzcomment{the Gaussian width is defined on the sample gradient set. Do we want to mention Gaussian width for population gradient? Also, do the results in 2.2 hold for population gradient as well? pending on proofs of Section 2.2}\abcomment{updated for now}
%
%\abcomment{para will be updated, maybe after we have the empirical results in Section 2.1 and theory in Section 2.2}

% \abcomment{from old Section 2 ... will need polish}
% \abbcomment{rewrite/edit/compress/drop this para; also, fix the notation -- TODO} 
% \yzdelete{For most deep learning models, under reasonable choices of $\Theta, \cZ$, one can show that for $\ggamma \in \Gamma$, $\| \ggamma \|_2 = O(1)$ whp (with high probability) w.r.t.~the randomness of the initialization \cite{du2018gradient,allen2019convergence,arora2019fine}. \yzcomment{double check if these citations are good.}} 
%\abcomment{old text} 

In this section, we initiate the study of loss gradient Gaussian width (LGGW) of deep learning gradients. As a warm up, we review that bounded $L_2$ norm, e.g., $\| \xi (\theta; z) \|_2 \leq c$ for any $\theta \in \Theta$ and $z \in \cZ$, with no additional structure, leads to a large Gaussian width since for such $\hat{\Xi}_n$, 
$w({\hat{\Xi}_n}) = \E_{\g}[\sup_{\hat{\xi}_n}\langle \hat{\xi}_n, \g \rangle ] \leq c \E_{\g}[ \langle \g/\|\g\|_2, \g\rangle ] = c \E_{\g}[\|\g\|_2] = O(\sqrt{p})$. We posit that the Gaussian width of deep learning gradients is much smaller and present a set of technical results in support. In Section~\ref{ssec:geometry}, motivated by the empirically observed sharp eigenvalue decay of loss Hessians, under mild assumptions we show that LGGW can be bounded by an upper bound on the $L_2$ norm of the Hessian eigenvalues, which has been empirically shown to be $\tilde{O}(1)$~\cite{zhang_why_2024,xie_power-law_2022}. Further, in Section~\ref{ssec:gwnn}, we show that under standard assumptions, the LGGW can be bounded in terms of the Gaussian width of the featurizer, i.e., output of the last-but-one layer, for both feedforward and residual networks. The results emphasize the benefits of Hessian eigenvalue decay and the stability of featurizers for deep learning.


%review empirical evidence and present examples based on such empirically observed geometry (), followed by precise derivations for FeedForward networks (FFNs) and residual networks (ResNets) (Section~\ref{ssec:gwnn}. Our results place $w({\hat{\Xi}_n})$ at anywhere between $\tilde{O}(1)$ to $\tilde{O}(\sqrt[4]{p})$, depending on the specific setting under consideration. 
%In modern deep learning, the largest models have approximately a trillion parameters, e.g., $p=10^{12}$. Consequently, our findings position the Gaussian width in the range of $20$ to $1000$, indicating its relatively diminutive scale. 
%A more thorough investigation of Gaussian width of deep learning gradients will be considered in future work.
%\abcomment{In modern deep learning, the largest models have about a trillion parameters, so that with $p=10^{12}$, our results place the Gaussian  width at $20$ to $1000$, hence small.} 


% \begin{figure*}[t] 
% \hspace*{-2mm}
% \centering
%  \subfigure[Sorted gradient coordinate absolute values (linear scale).]{
%   % [trim=left bottom right top, clip]
%  \includegraphics[trim = 1mm 1mm 1mm 4mm, clip, width=0.22\textwidth]{figs/top_gt_mnist_linear.png}
%  } % \vspace{-2mm}
%  \hspace*{1mm}
%  \subfigure[Sorted gradient coordinate absolute values (log scale).]{
%  \includegraphics[trim =1mm 1mm 1mm 4mm, clip, width=0.22\textwidth]{figs/top_gt_mnist_log.png}
%  } % \vspace{-2mm}
%   \subfigure[Sorted gradient coordinate absolute values (linear scale).]{
%   % [trim=left bottom right top, clip]
%  \includegraphics[trim = 1mm 1mm 1mm 4mm, clip, width=0.22\textwidth]{figs/top_gt_cifar_linear.png}
%  } % \vspace{-2mm}
%  \subfigure[Sorted gradient coordinate absolute values (log scale).]{
%   % [trim=left bottom right top, clip]
%  \includegraphics[trim = 1mm 1mm 1mm 4mm, clip, width=0.22\textwidth]{figs/top_gt_cifar_log.png}
%  } % \vspace{-2mm}
% \caption{(a-b) Sorted gradient coordinate in linear scale (a) and log scale (b) for SGD over 100 epochs on CIFAR-10.
% %batch size 128, learning rate 0.01, averaged over 5 runs. 
% Model: 4-hidden-layer ReLU network with 256 nodes on each layer, with around 1,055,000 parameters. (c-d) Sorted gradient coordinate in linear scale (c) and log scale (d) for SGD over 100 epochs on MNIST. Model: 2-layer ReLU with 128 nodes on each layer, with roughly 120,000 parameters. Y-axis is the absolute value of gradient coordinates, X-axis is sorted in increasing order. }
% \vspace*{-3mm}
% \label{fig:cifar_eva}
% \end{figure*}

% \begin{figure*}[t] 
% \centering
%  \subfigure[SGD]{
%   % [trim=left bottom right top, clip]
%  \includegraphics[trim = 3mm 1mm 4mm 4mm, clip, width=0.30\textwidth]{figs/eva_mnist_sgd.png}
%  } % \vspace{-2mm}
%   \subfigure[DP-SGD, $\sigma = 1.0$]{
%  \includegraphics[trim =3mm 1mm 4mm 4mm, clip, width=0.30\textwidth]{figs/eva_mnist_dpsgd_no1.png}
%  } % \vspace{-2mm}
%  \subfigure[DP-SGD, $\sigma = 2.0$]{
%   % [trim=left bottom right top, clip]
%  \includegraphics[trim = 3mm 1mm 4mm 4mm, clip, width=0.30\textwidth]{figs/eva_mnist_dpsgd_no2.png}
%  }
%  \vspace{-3mm} 
% \caption[]{Top 500 eigen-value spectrum of the gradient second moment matrix along the training trajectory of SGD, DP-SGD with noise variance $\sigma=1, 2$. Dataset: MNIST; model: 2-layer ReLU with 128 nodes each layer. The network has roughly 130,000 parameters and is trained on MNIST dataset. The Y-axis is the eigenvalue and X-axis is order of eigenvalues from largest to smallest.}
% \vspace{-4mm}
% \label{fig:mnist_eva}
% \end{figure*}
%\vspace{-2mm}


\subsection{Loss Gradient Gaussian Width using Empirical Eigen Geometry of Hessian}
\label{ssec:geometry}
In the context of deep learning, recent work has illustrated that empirically the gradients are considerably structured and gradients are effectively live in a low-dimensional space~\cite{gur-ari_gradient_2018,papyan_full_2018,papyan_measurements_2019,ghorbani_investigation_2019,lgzcb20}, and
%and during optimization, the gradients are ``simple'' in the sense that the sorted absolute gradient components decay quickly and the components have large values only for a small subset of parameters (e.g., see Figure~\ref{fig:cifar_eva}),
% the eigen-spectrum of the gradient outer product matrix over epochs has a sharply decaying eigenvalues (e.g., see Figure~\ref{fig:cifar_eva} (c)); 
 close to convergence, almost all gradients are really close to zero, the so-called interpolation condition~\cite{bhmm19,negrea_defense_2019,ma_power_2017,bartlett_[1906.11300]_2019}. 
Such observations have formed the basis of more memory or communication-efficient algorithms, e.g., based on top-$k$ count-sketch, truncated SGD, and heavy hitters based analysis~\cite{rothchild2020fetchsgd,ivkin2019communication}. In parallel, considerable advances have been made in understanding the eigenspectrum of the Hessian~\cite{zhang_why_2024,xie_power-law_2022,yao_pyhessian_2020,li2020hessian}. In particular, fast decaying eigenvalues have been observed across the entire range of models including ConvNets, ResNets, as well as GPT and ViT variants~\cite{zhang_why_2024,yao_pyhessian_2020}, and some work~\cite{xie_power-law_2022} have empirically shown that the $k$-th largest (absolute) eigenvalue decays following power-law, i.e., $\lambda_k \leq \lambda_1 k^{-s}$ with $s > \frac{1}{2}$ empirically. 
%The sharp eigenvalue decay of the Hessian also explains the observed properties of the gradients [][]. 

We make some assumptions based on the empirically observed eigenvalue decay of the Hessian and establish bounds on the loss gradient Gaussian width based on properties of the Hessian eigenvalues.
\begin{asmp}
Let $\hat H_n(\theta) = \frac{1}{n} \sum_{i=1}^n \nabla^2 \ell(\theta, z_i)$ denote the loss Hessian for $\theta \in \Theta$ and let $\llambda(\theta) = [\lambda_i(\theta)], i \in[p]$ denote the (not necessarily positive) eigenvalues of $\hat H_n(\theta)$. For any $\theta \in \Theta$, the empirical gradient $\hat \xi_n(\theta) = \hat H_n(\tilde{\theta}) (\theta - \theta_0) + \hat \xi_n(\theta_0)$ for some $\theta_0 \in \R^p, \| \theta - \theta_0 \|_2 \leq c$, where $\tilde{\theta} = a_{\theta} \theta + (1-a_{\theta}) \theta_0, a_{\theta} \in [0,1]$. With $\llambda(\tilde{\theta})$ 
denoting the Hessian eigenvalues of $\hat H_n(\tilde{\theta})$ at any such $\tilde{\theta}$, we assume $\left\|\llambda(\tilde{\theta})\right\|_{2}\leq\Lambda^{(u)}$ 
%\left\|\llambda^{(u)} \right\|_{2}$
%$|\lambda_{(i)}(\tilde{\theta})| \leq \lambda^{(u)}_{(i)}, i \in [p]$ 
for some fixed $\Lambda^{(u)} \in \R_+$.
%\llambda^{(u)} \in \R^p$. 
%\item There exists $\theta_0 \in \R^p$ such that for $\theta \in \Theta, \| \theta - \theta_0 \|_2 \leq c$.
%\item For any $\theta \in \Theta$, the gradient $\xi(\theta) = \hat H_n(\tilde{\theta}) (\theta - \theta_0) + \xi(\theta_0)$ for some $\theta_0 \in \Theta_0 \subset \R^p$ and $\|\theta - \theta_0\| \leq c$, where $\tilde{\theta} = a_{\theta} \theta + (1-a_{\theta}) \theta_0, a_{\theta} \in [0,1]$. \vspace{-3mm}
%, with $(i)$ denoted the $i$-th largest (absolute) value. 
%\end{enumerate}
\label{asmp:eigdecay}
\end{asmp}


% \begin{asmp}
% Let $\hat H_n(\theta) = \frac{1}{n} \sum_{i=1}^n \nabla^2 \ell(\theta, z_i)$ denote the loss Hessian for $\theta \in \Theta$ and let $\llambda(\theta) = [\lambda_i(\theta)], i \in p$ denote the (not necessarily positive) eigenvalues of $\hat H_n(\theta)$. 
% \begin{enumerate}[(a)]
% \item For any $\theta \in \Theta$, the gradient $\xi(\theta) = \hat H_n(\tilde{\theta}) (\theta - \theta_0) + \xi(\theta_0)$ for some $\theta_0 \in \Theta_0 \subset \R^p$ and $\|\theta - \theta_0\| \leq c$, where $\tilde{\theta} = a_{\theta} \theta + (1-a_{\theta}) \theta_0, a_{\theta} \in [0,1]$.
% \item With $\llambda(\tilde{\theta})$ denoting the Hessian eigenvalues of $\hat H_n(\tilde{\theta})$ at $\tilde{\theta}$, we have $\left\|\llambda(\tilde{\theta})\right\|_{2}\leq\left\|\llambda^{(u)} \right\|_{2}$
% %$|\lambda_{(i)}(\tilde{\theta})| \leq \lambda^{(u)}_{(i)}, i \in [p]$ 
% for some fixed $\llambda^{(u)} \in \R_+^p$.
% %, with $(i)$ denoted the $i$-th largest (absolute) value. 
% \end{enumerate}
% \label{asmp:eigdecay}
% \end{asmp}
% \qlcomment{I think (a) is indeed coming from the mean-value theorem for vector functions, and we might only need the $\ell_{2}$ norm is bounded by a constant vector instead of a coordinate-wise bound.}

\begin{remark}
Assumption~\ref{asmp:eigdecay} is inspired by the empirical evidence of Hessian eigenvalue decay especially close to convergence~\cite{zhang_why_2024,xie_power-law_2022}, and it is reasonable to expect $\left\|\lambda(\tilde{\theta})\right\|_{2}=\tilde{O}(1)$, which means we could set $\Lambda^{(u)}=\tilde{O}(1)$. %\|\llambda^{(u)} \|_2 = \tilde{O}(1)$. 
In Assumption~\ref{asmp:eigdecay}, $\theta_0$ can be from a pretrained model or a random initialization. Further, we can replace the single $\theta_0$ by a set $\Theta_0$ of cardinality $|\Theta_0|=N$, so that for any $\theta \in \Theta, \exists \theta_0 \in \Theta_0$ such that $\| \theta - \theta_0 \|_2 \leq c$, and our main result below will continue to hold with only an additional $\log N$ term~\cite{maurer_inequality_2014,chba15}. \qed    
\end{remark}
%Note that $\theta_0$ can (a) follows from mean-value theorem, and we allow a set $\Theta_0$ of cardinality $N$, i.e., $|\Theta_0| = N$, so a ``nearby'' $\theta_0$ can be found for any $\theta \in \Theta$. Our width bound will only have a $\log N$ dependence. Further, (b) is motivated from the empirically observed sorted eigenvalue decay ideally implying $\lambda^{(u)}_{(i)}$ also decays reasonably quickly. 

\begin{restatable}{theo}{eigdecay}
Under Assumption~\ref{asmp:eigdecay}, the LGGW for $\theta \in \Theta$ is $w(\hat{\Xi}_n)\leq c\Lambda^{(u)}\sqrt{\log p}$.%\| \llambda^{(u)} \|_2 \sqrt{\log p}$.
\label{lemm:eigdecay}
\end{restatable}
\begin{remark}
The width bound in Theorem~\ref{lemm:eigdecay} depend on $\Lambda^{(u)}$, the upper bound of $\left\|\llambda(\tilde{\theta})\right\|_{2}$, 
%\| \llambda^{(u)} \|_2$, 
so that a power law decay of sorted absolute Hessian eigenvalues $|\lambda_{(i)}(\tilde{\theta})| \leq c^{(u)} i^{-s}$ with $s \geq \frac{1}{2}$ (e.g., as empirically observed in~\cite{xie_power-law_2022}) will lead to $\Lambda^{(u)} = O(\sqrt{\log p})$. Then, the overall bound is $w(\hat{\Xi}_n) \leq c \log p$ yielding a generalization bound from \eqref{eq:genbndex} with complexity term $c \frac{\log p}{\sqrt{n}}$, hence a sharp bound. \qed 
\end{remark}


%
% Under suitable assumptions on the population gradient geometry based on these empirical observations such as low-rank gradient structure and decaying gradient components, we outline concrete versions of upper bounds on the Gaussian width of gradients. We illustrate that in such scenarios, the Gaussian width exhibits at most a logarithmic dependence on the dimensionality $p$. We establish bounds on the Gaussian width in the following examples, using $c_i$ to represent absolute constants. 
%
% \abdelete{
% \abcomment{the following bit is currently floating -- include somewhere, move to appendix, or drop} We augment these empirical observations with some examples of gradient sets which have small Gaussian widths by construction or by suitable composition properties.
% %~\cite{tala14,vers18}. 
% \begin{exam}[\bf{Ellipsoid}]
% Consider $\hat{\Xi}_n = \{ \hat{\xi}_n \in \R^p \mid \sum_{j=1}^p ((\hat{\xi}_n[j])^2/a_j^2 = \tilde{O}(1), a \in \R^p\}$.
% %where $\tilde{O}$ hides polylog$(p)$ terms. 
% Then, the Gaussian width $w(\hat{\Xi}_n) = \tilde{O}(\| \a \|_2)$~\cite{tala14}. Note that if $\| \a \|_2 = \tilde{O}(1)$, then we have $w(\hat{\Xi}_n) = \tilde{O}(1)$. For example, if the elements of $\a$ sorted in decreasing order satisfy $a_{(j)} \leq c_3/\sqrt{j}$, then $\|\a\|_2 = \tilde{O}(1)$. \qed 
% %for this ellipsoid, a sufficient condition is for the sorted gradient components to satisfy $\gamma_{(j)} \leq a_{(j)}/\sqrt{j} \leq c_3/j$. \qed 
% \label{exm:ellipsoid}
% \end{exam}
% %
% % \begin{exam}[{\bf Small ball}]
% % \abcomment{drop this example?} An interesting special case of the ellipsoid example is the following: if the elements of $a$ sorted in decreasing order satisfy $a_{(j)} \leq c_3/j$, then $\| a\|_2 \leq \frac{c_3\pi}{\sqrt{6}}$, so that  $\gamma_2(\cM,\| \cdot \|_2) \leq c_4 \frac{\pi}{\sqrt{6}}$, which is a constant independent of $p$.
% % \label{exm:small}
% % \end{exam}
% %
% \begin{exam}[\bf{$k$-support norm}]
% The $k$-support norm 
% $$\|\xi\|_k^{sp} = \inf_{\sum_i u_i = \xi}\left\{ \sum_i \| u_i \|_2 \mid \| u_i \|_0 \leq k\right\} \vspace*{-2mm}$$ 
% is based on an infimum convolution over $k$-sparse vectors~\cite{agfs12,mcps14,chba15}, with $k=1$ corresponding to the $L_1$ norm. Consider $\hat{\Xi}_n = \{ \hat{\xi}_n \mid \|\hat{\xi}_n\|_k^{sp} \leq c_0 \sqrt{k} \}$. Note that among many other things $\hat{\Xi}_n$ includes 
% the infimum convolution of all $k$-sparse gradients $\hat{\xi}_n$ with each non-zero element bounded by $c_0$. By construction, $w(\hat{\Xi}_n) \leq c_1 k \sqrt{\log (p/k)}$~\cite{chba15}. \qed
% \label{exm:ksupport}
% \end{exam}
% %
% \begin{exam}[{\bf Union of sets}]
% If $\hat{\Xi}_n$ is an union of $p^r$ sets, i.e., polynomial in $p$, where each set has a $\tilde{O}(1)$ Gaussian width and each element has $\tilde{O}(1)$ $L_2$ norm, then $w(\hat{\Xi}_n) = \tilde{O}(\sqrt{r})$~\cite{mapr14,chba15}. Taking convex hull of such $\hat{\Xi}_n$ can only change its Gaussian width by a constant amount, i.e., $w(\text{conv}(\hat{\Xi}_n)) \leq c_2 w(\hat{\Xi}_n)$~\cite{tala14}(Theorem 2.4.15). \qed
% \label{exm:union}
% \end{exam}
% %
% \begin{exam}[{\bf Minkowski sum of sets}]
% If $\hat{\Xi}_n$ is Minkowski sum of a union of $p^r$ sets as in Example~\ref{exm:union} and a $\sqrt{k}$ radius $k$-support norm ball as in Example~\ref{exm:ksupport}, then $w(\hat{\Xi}_n) = \max(k,\sqrt{r})\tilde{O}(1)$. \qed 
% \end{exam}
% \vspace{-2mm}
% Based on how the gradients empirically look for deep networks (Figures~ \ref{fig:cifar_eva}), it is arguably fair to assume that the gradients live in $\hat{\Xi}_n$ with small Gaussian width. We prove explicit upper bound of $w(\hat{\Xi}_n)$ for FFNs  and ResNets in Sections~\ref{ssec:ffn} and \ref{ssec:resnet} respectively)
% }
% \abbcomment{polish or drop -- TODO} 
% \yzdelete{Based on how the gradients empirically look like for deep networks (Figures~ \ref{fig:cifar_eva} (a) - (c)), it is arguably fair to assume that the gradients live in $\hat{\Xi}_n$, a convex hull of a Minkowski sum of (a) union of $p^r$, i.e., polynomially many ellipsoids, each with $\|\a\|_2 = \tilde{O}(1)$ and (b) a $k$-support norm ball of radius $O(\sqrt{k})$. For such a set, we have $w(\hat{\Xi}_n) = \tilde{O}(\max(\sqrt{r},k) \log p)$. In the next two sections, we prove such upper bounds for \emph{feed-forward networks} and \emph{residual networks} (Sections~\ref{ssec:ff} and \ref{ssec:resnet} respectively) under standard modeling assumptions. }




\subsection{Gaussian Width Bounds for Neural Networks}
\label{ssec:gwnn}

Consider a training set $z^{(n)} = \{z_i, i \in [n]\}, z_i=(\x_i,y_i), \x_i \in \cX \subseteq \R^d, y_i \in \cY \subseteq \R$.
%\yzcomment{we used $z^{(n)}$ as the finite samples and $z = (x, y)$ for individual sample. Shall we keep the notation consistent?}\abcomment{done}. 
% \abdelete{We will denote by $X\in\R^{n\times d}$ the matrix whose $i$-th row is $\x_i^\top$.} 
For some loss function $l$, the goal is to minimize:   $\hat \cL_n(\theta)  = \frac{1}{n} \sum_{i=1}^n l(  y_i, \hat{y}_i) = \frac{1}{n} \sum_{i=1}^n l (y_i,f(\theta;\x_i))$, where the prediction $\hat{y}_i:= f(\theta;\x_i)$ is from a neural network, and the parameter vector $\theta\in\R^p$. 
%As in modern neural networks, we will assume $p$ to be large.
% \abdelete{In terms of the notation, $l(y_i,f(\theta;\x_i)) \equiv \ell(\theta,z_i)$, and our usage will depend on the context.}
%
% \abdelete{Consider the pointwise loss $l_i:=l(y_i,\cdot) : \R \to \R_+$ and denote its first-derivative as $l'_i := \frac{d l(y_i,\hat{y}_i)}{d \hat{y}_i}$.}
% For the particular case of square loss, $l(y_i,\hat{y}_i)=\frac{1}{2}(y_i-\hat{y}_i)^2$. 
% We denote the gradient of the predictor $f(\cdot;\x_i):\R^p \to \R$ as
% $\nabla_i f := \frac{\partial f(\theta;\x_i)}{\partial \theta}$. 
% %
% The gradient of the empirical loss $\hat \cL_n(\theta) = \frac{1}{n} \sum_{i=1}^n l(y_i,f(\theta,\x_i))$ is given by
% %\begin{align}
% $\frac{\partial\hat \cL_n(\theta)}{\partial \theta}  
% = \frac{1}{n} \sum_{i=1}^n l_i' \nabla_i f 
% =  \frac{1}{n} \sum_{i=1}^n l_i' \frac{\partial f(\theta;\x_i)}{\partial \theta}$.
%\end{align}
For our analysis, we will assume square loss $l(y_i,\hat{y}_i)=\frac{1}{2}(y_i-\hat{y}_i)^2$, 
%i.e., $l_i(\theta) :=  (y_i - f(\theta;x_i))^2$, 
though the analyses extends to more general losses under mild additional assumptions.
%e.g., $|l'_i|=O(1)$. 
%We also make standard scaling assumptions: $\|\x_i\|_2 \leq \sqrt{d}, |y_i|=O(1)$.
%
% We work with Feed-Forward Networks (FFNs) in Section~\ref{ssec:ffn} and ResNets in Section~\ref{ssec:resnet}. 
We focus on feedforward networks (FFNs) and residual networks (RestNets), and consider them as $L$ layer neural networks $f(\theta;\x)$ with parameters $\theta$, where each layer has width $m$. 
% \abdelete{where the parameter $\theta \in \R^p, p = m^2(L-1) + md + m$ constitutes of $L$ layerwise matrices $W^{(l)}$ and one vector $\v \in \R^m$ for the last layer. }
We make two standard assumptions~\cite{allen-zhu_convergence_2019,du_gradient_2019,liu_linearity_2021,banerjee_rsc23}.
%for the analysis for both FFNs and ResNets.
\begin{asmp}[{\bf Activation}]
The activation function $\phi$ is 1-Lipschitz, i.e., $|\phi'| \leq 1$ and $\phi(0) = 0$.
\label{asmp:act}
\end{asmp}
\begin{asmp}[\bf{Random initialization}]
Let $\theta_0 := (\vec(W_0^{(1)})^\top,\ldots,\vec(W_0^{(L)})^\top, \v_0^\top )^\top 
%\in \R^{\sum_{k=1}^L m_k m_{k-1}+m_{L}}
$ denote the initial weights, and   $w_{0,ij}^{(l)}$ denote $i, j$-th element of weight matrix $W_0^{(l)}$ for $l\in[L]$.
At initialization, $w_{0,ij}^{(l)} \sim \cN(0,\sigma_0^{(l)}{}^2)$ for $l\in[L]$ where $\sigma_{0}^{(1)}=\frac{\sigma_{1}}{2\left(1+\frac{\log m_{1}}{2m_{1}}\right)}$, $\sigma_0^{(l)} = \frac{\sigma_1}{1 + \sqrt{\frac{m_{l-1}}{m_{l}}}+\sqrt{\frac{2\log m_{l}}{m_{l}}}}$, $l\geq2$, $\sigma_1 > 0$, and 
%$\v_0$ is a random unit vector with 
$\norm{\v_0}_2=1$. 
\label{asmp:ginit}
\end{asmp}
Assumption \ref{asmp:act} is satisfied by commonly used activation functions such as (non-smooth) ReLU \cite{allen2019convergence} and (smooth) GeLU \cite{hendrycks2016gaussian}. %\abdelete{Our analysis goes through without these assumptions with suitable modifications, \abedit{as discussed in the sequel} \abcomment{(or drop this part??)}.}
%
And Assumption \ref{asmp:ginit} is regarding the random initialization of the weights, variants of which are typically used in most work in deep learning theory \cite{jacot_neural_2020, allen2019convergence,he2015delving,glorot2010understanding,sutskever2013importance,arora2019fine,du2018gradient,du_gradient_2019}.  


% \yzcomment{clarification on $r$}\abcomment{made $r=2$ to simplify things}

% \abcomment{if we work out the uniform random initialization case, we will add it here}\yzcomment{good idea}

%\yzcomment{finished reading and editing up to this point}
%\yzcomment{the loss gradient set up is not used anywhere.}

\subsubsection{Bounds for FeedForward Networks (FFNs)}
\label{ssec:ffn}

We consider $f$ to be an FFN given by 
\begin{equation}   
f(\theta;x) = \v^\top \phi(\frac{1}{\sqrt{m_{L}}}W^{(L)} \phi(\cdots \phi( \frac{1}{\sqrt{m_{1}}}  W^{(1)} \x))))~,
\label{eq:ffn}    
\end{equation}
where $W^{(1)} \in \R^{m \times d}, W^{(l)} \in \R^{m_{l} \times m_{l-1}}, l \in \{2,\ldots,L\}$ are the layer-wise weight matrices, $\v\in\R^{m_{L}}$ is the last layer vector, $\phi(\cdot )$ is the (pointwise) activation function, and the total set of parameters $\theta \in \R^{p}, p=\sum_{k=1}^{L}m_{k}m_{k-1}+m_{L}$ is given by
\begin{align}
\theta = (\vec(W^{(1)})^\top,\ldots,\vec(W^{(L)})^\top, \v^\top )^\top.
\label{eq:theta_def}
\end{align}
in which $m_{0}=d$.
%
Our analysis for both FFNs and ResNets will be for gradients over all parameters in a fixed radius {\em spectral} norm ball around the initialization $\theta_0$, which is more flexible than Frobenius norm balls typically used in the literature \cite{woodworth_kernel_2020,chizat_lazy_nodate,zou_stochastic_2018,banerjee_rsc23}:
%\vspace{-2mm}
\begin{equation}
%\begin{split}
B_{\rho, \rho_1}^{\spec}(\theta_0) := \big\{ \theta \in \R^p ~\text{as in \eqref{eq:theta_def}} ~\mid  \| \v - \v_0 \|_2 \leq \rho_1,   \|W^{(\ell)} - W_0^{(\ell)} \|_2 \leq \rho, \ell \in [L]  \big\} 
\label{eq:specball} ~.
%\end{split}
\end{equation}
Let $B_{\rho}^{\spec}(\theta_0) \in \R^{p-m}$ be the corresponding set of weight matrices $W = \{W^{(l)}, \ell \in [L]\}$. The main implications of our results and analyses go through as long as the layerwise spectral radius $\rho = o(\sqrt{m})$ and last layer radius $\rho_1 = O(1)$, which are arguably practical. 

Let 
% $h^{(L)}(W,\x)  := \phi\left(\frac{1}{\sqrt{m}}W^{(L)} \phi(\cdots \phi( \frac{1}{\sqrt{m}}  W^{(1)} \x))) \right) ~\in \R^m$
\begin{align}
h^{(L)}(W,\x) & := \phi\left(\frac{1}{\sqrt{m_{L}}}W^{(L)} \phi(\cdots \phi( \frac{1}{\sqrt{m_{1}}}  W^{(1)} \x))) \right) ~\in \R^{m_{L}}
\end{align}
be the ``featurizer,'' i.e., output of the last but one layer, so that $f(\theta;\x) = \v^\top h^{(L)}(W,\x)$ with $\theta = (W,\v)$. Consider the set of all featurizer values for a single sample and as average over samples:
\begin{align}\label{eq:feature_set}
A^{(L)}(\x) = \left\{ h^{(L)}(W,\x) \mid W \in B_{\rho}^{\spec}(\theta_0) \right\},~ \hat{A}_n^{(L)} := \left\{ \frac{1}{n} \sum_{i=1}^n h^{(L)}(W,\x_i) \mid W \in B_{\rho}^{\spec}(\theta_0) \right\} ~.
\end{align}  

We now establish an upper bound on the LGGW of FFN gradient set $\hat{\Xi}_{n}^{\ffn}$ corresponding to parameters in $B_{\rho, \rho_1}^{\spec}(\theta_0)$. In particular, we show that the LGGW can effectively be bounded by the Gaussian width of the sample average of the featurizer.
\begin{restatable}[\bf{Gaussian Width of Gradients: FFNs}]{theo}{theofnngradwidth}
\label{cor:gradient-bounds}
Under Assumptions~\ref{asmp:act} and \ref{asmp:ginit}, with $\beta_{l} := \sigma_1 + \frac{\rho}{\sqrt{m_{l}}}$, $l\in[L]$, with probability at least $\left(1-\sum_{l=1}^{L}\frac{2}{m_{l}}\right)$ over the randomness of the initialization, we have
\begin{align}
w(\hat{\Xi}_n^{\ffn}) \leq c_{1}w(\hat{A}_{n}^{(L)})+c_{2}(1+\rho_{1})\sqrt{m_{L}}\prod_{l=1}^{L}\beta_{l}\sum_{l=1}^{L}\frac{1}{\beta_{l}\sqrt{m_{l}}}~. 
\end{align}
\end{restatable}

\begin{remark}
For the simplest case, with $m_{l}=m$ for all $l\in[L]$, we have that
\begin{align*}
    w(\hat{\Xi}_n^{\ffn}) \leq c_1 w(\hat{A}_{n}^{(L)} ) + c_2 L(1+\rho_{1}) \beta^{L-1}~. 
\end{align*}
in which $\beta = \sigma_{1}+\frac{\rho}{\sqrt{m}}$. Note that choosing $\sigma_1 < 1 - \frac{\rho}{\sqrt{m}}$, i.e., mildly small initialization variance, satisfies $\beta < 1$. When $\beta < 1$, we have $w(\hat{\Xi}_n^{\ffn}) = O(1)$ as long as $L = \Omega ( \frac{\log (\sqrt{m} + L(1+\rho_{1}))}{\log \frac{1}{\beta}} )$,
% \abmargincomment{check, clean-up}, 
which holds for moderate depth $L$. To see this, note that we have $w(\hat{\Xi}_n^{\ffn}) = O(w(\hat{A}^{(L)}_n) + L (1+\rho_{1})\beta^{L-1})$.  Further, we have whp $\| \alpha^{(L)} \|_2 \leq \beta^L$ (Lemma~\ref{lemma:layer} in Appendix~\ref{app:gauss_width}), so that $w(\hat{A}^{(L)}_n) \leq c \beta^L \sqrt{m}$. Then, for $\beta < 1$, the bound $\beta^L \sqrt{m} + \beta^{L-1} L(1+\rho_{1}) = O(1)$ if $L = \Omega ( \frac{\log (\sqrt{m} + L(1+\rho_{1}))}{\log \frac{1}{\beta}} )$. Interestingly, sufficient depth $L$ helps control the Gaussian width in the theoretical setting. \qed 
\end{remark}
\begin{remark}
In practice, the dimensions of the hidden layers $m_{l}, l\in[L-1]$ are always much larger than the dimension of the output layer $m_{L}$, and our bound is even better under such situations. First, for the high probability,
\begin{align*}
    1-\sum_{l=1}^{L}\frac{2}{m_{l}}\gg1-\frac{2L}{m_{L}}.
\end{align*} 
Second, for the bound with respect to the parts other than the featurizer,
\begin{align*}
    \left(1+\rho_{1}\right)\sqrt{m_{L}}\prod_{l=1}^{L}\beta_{l}\sum_{l=1}^{L}\frac{1}{\beta_{l}\sqrt{m_{l}}}\ll L\left(1+\rho_{1}\right)\beta_{L}^{L-1}
\end{align*}
Therefore, both the probability and the bound are much sharper.
\qed
\end{remark}
Technicalities aside, Theorem~\ref{cor:gradient-bounds} has two qualitative implications which are important to understand.
\begin{remark}
Theorem~\ref{cor:gradient-bounds} bounds the Gaussian width uniformly over all parameters in $B_{\rho,\rho_1}^{\spec}(\theta_0)$. Instead, we can consider the bound for parameters in $\Theta$ which are in the last 10\% of the epochs of deep learning training. If the featurizer for such parameters $\theta \in \Theta$ are more stable, i.e., does not change much with changes in $W$, then the Gaussian width of the featurizer will be small. \qed 
\end{remark}
\begin{remark}
The result implies that under suitable conditions, the Gaussian width of gradients over all $p = \sum_{k=1}^{d}m_{k}m_{k-1}+m_{L}$ parameters can be reduced to the Gaussian width of the featurizer, which is $m_{L}$ dimensional. If the featurizer does feature selection, e.g., as in variants of invariant risk minimization (IRM)~\cite{arjovsky_invariant_2020,zhou_sparse_2022} or sharpness aware minimization (SAM)~\cite{foret_sharpness-aware_2021,andriushchenko_sharpness-aware_2023}, then the Gaussian width of the featurizer will be small. On the other hand, if the featurizer has many spurious and/or random features~\cite{rosenfeld_risks_2021,zhou_sparse_2022}, then the Gaussian width will be large. \qed 
\end{remark}

% \yzcomment{1. how do we get $L = \Omega(\frac{\log m}{\log \frac{1}{\beta}})$?\\
% 2. how do we know $\rho$ in practice? or we say one can constrain the weight in such a spectral norm ball around the initialization during training? }
\begin{figure}[t]
    \centering
    \begin{subfigure}[b]{0.3\textwidth}
        \includegraphics[width=\textwidth]{arXiv_v2/figures/Featurizer/l0_l1_norms-updated.png}
        \caption{ResNet18 on CIFAR-10}
        \label{fig:resnet18_cifar10_feature}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.3\textwidth}
        \includegraphics[width=\textwidth]{arXiv_v2/figures/Featurizer/l0_l1_norms-updated-ffn.png}
        \caption{FFN on CIFAR-10}
        \label{fig:ffn_cifar10_feature}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.3\textwidth}
        \includegraphics[width=\textwidth]{arXiv_v2/figures/Featurizer/l0_l1_norms-updated-cf.png}
        \caption{CNN on Fashion-MNIST}
        \label{fig:cnn_fashion_mnist_feature}
    \end{subfigure}
    \caption{$L_{0}$ norm and $L_{1}$ norm of featurizers for (a) ResNet18 on CIFAR-10, (b) FFN on CIFAR-10, and (c) CNN on Fashion-MNIST of the last 10\% epochs close to convergence. We plot both the average and maximum norms among 5 repetitions for each experiment. The figures demonstrate that for these models, as approaching convergence, the featurizers has relatively low $L_{0}$ norm and $L_{1}$ norm, which further indicates a small LGGW. All experiments are run on A100 GPUs.}
    \label{fig:featurizer-norms}
\end{figure}
\subsubsection{Bounds for Residual Networks (ResNets)}
\label{ssec:resnet}

We consider $f$ to be a ResNet  given by 
% $\alpha^{(l)}(\x)  =  \alpha^{(l-1)}(\x) + \phi \left( \frac{1}{L \sqrt{m}} W^{(l)} \alpha^{(l-1)}(\x) \right)$ and $f(\theta;\x)  = \alpha^{(L+1)}(\x)  = \frac{1}{\sqrt{m}} \v^\top \alpha^{(L)}(\x)$,
% \abcomment{notation is not entirely consistent with the previous section, where $\alpha^{(L)}(W,x)$ denoted the featurizer}
\begin{equation}
\begin{split}
 \alpha^{(l)}(\x)  & =  \alpha^{(l-1)}(\x) + \phi \left( \frac{1}{L \sqrt{m_{l}}} W^{(l)} \alpha^{(l-1)}(\x) \right)~,\\%~~~l \in [L]~,\\
f(\theta;\x) & = \alpha^{(L+1)}(\x)  = \v^\top \alpha^{(L)}(\x)~,
\end{split}
\label{eq:resnet}    
\end{equation}
where $\alpha^{(0)}(\x) = \x$, and $W^{(l)}, l \in [L], \v, \phi$ are as in FFNs. Let $h^{(L)}(W,\x)  := \alpha^{(L)}(\x)$ be the ``featurizer,'' i.e., output of the last layer, so that $f(\theta;\x) = \v^\top h^{(L)}(W,\x)$ with $\theta = (W,\v)$.
Note that the scaling of the residual layers is assumed to have a smaller scaling factor $\frac{1}{L}$ following standard theoretical analysis of ResNets~\cite{du_gradient_2019} and also aligns with practice where smaller initialization variance yields state-of-the-art performance~\cite{zhang_understanding_2017}.
With the featurizer and associated sets defined as in \eqref{eq:feature_set} for FFNs, we now establish an upper bound on the LGGW of gradients in terms of that of the featurizer.
\begin{restatable}[\bf{Gaussian Width of Gradients: ResNets}]{theo}{theorngradwidth}
\label{cor:gradient-bounds-resnet}
Under Assumptions~\ref{asmp:act} and \ref{asmp:ginit}, with $\beta_{l} := \sigma_1 + \frac{\rho}{\sqrt{m_{l}}}$, $l\in[L]$, with probability at least $\left(1-\sum_{l=1}^{L}\frac{2}{m_{l}}\right)$ over the randomness of the initialization,  we have
\begin{align}
w(\hat{\Xi}_n^{\resnet}) \leq c_{1}w(\hat{A}_{n}^{(L)})+c_{2}\frac{1+\rho_{1}}{L}\sqrt{m_{L}}\prod_{l=1}^{L}\left(1+\frac{\beta_{l}}{L}\right)\sum_{l=1}^{L}\frac{1}{\left(1+\frac{\beta_{l}}{L}\right)\sqrt{m_{l}}}~.
\end{align}
\end{restatable}
\begin{remark}
For the simplest case, with $m_{l}=m$ for all $l\in[L]$, we have that
\begin{align*}
    w(\hat{\Xi}_n^{\resnet}) \leq c_1 w(\hat{A}_n^{(L)}) + c_{2}\frac{1+\rho_{1}}{L}\left(1+\frac{\beta}{L}\right)^{L-1}\leq c_1 w(\hat{A}_n^{(L)}) + c_2 \frac{(1+\rho_{1})e^{\beta}}{L}~.
\end{align*}
in which $\beta = \sigma_{1}+\frac{\rho}{\sqrt{m}}$, and the second inequality holds since $\left(1+\frac{\beta}{L}\right)^{L-1}\leq e^{\beta}$. As for FFNs, choosing $\sigma_1 < 1 - \frac{\rho}{\sqrt{m}}$, i.e., mildly small initialization variance, satisfies $\beta < 1$. When $\beta < 1$, we have $w(\hat{\Xi}_n^{\resnet}) = O( w(\hat{A}_n^{(L)}) )$ since $(1+\rho_{1})e^\beta = O(1)$. Thus, for ResNets, the Gaussian width of gradients on all parameters reduces to the Gaussian width of the featurizer.  \qed 
\end{remark}
\begin{remark}
As for FFNs, our ResNet bound is also much sharper when the dimensions in the hidden layers are much larger than the output dimension, which is the case in commonly used ResNet models. 
\qed
\end{remark}
\begin{remark}
%In practice, for ResNets using ReLU activation, few of the features are empirically active close to convergence. 
In Figure \ref{fig:featurizer-norms}, we plot the average and max (over 5 runs) of the $L_0$ and $L_{1}$ norm of the featurizer for the last $10\%$ epochs close to convergence for three standard deep learning models: ResNet18 on CIFAR-10 (512 dimension featurizer), FFN on CIFAR-10 (256 dimension featurizer), and CNN on Fashion-MNIST (128 dimension featurizer). 
%From either small $L_{1}$ norms, small $L_{1}$ norms of the difference, or small $L_{0}$ norm, one can demonstrate 
%Such sparse featurizer implies 
The small $L_0$ and $L_1$ norm of the featurizer, indicating both feature selection and being in small $L_1$ ball, imply small Gaussian width of the featurizer which in turn implies small LGGW based on Theorems~\ref{cor:gradient-bounds} and \ref{cor:gradient-bounds-resnet}.
\qed  
\end{remark}

% Similarly, algorithms which implicitly or explicitly does feature selection on the featurizer, e.g., as in variants of invariant risk minimization (IRM)~\cite{arjovsky_invariant_2020,zhou_sparse_2022} or sharpness aware minimization (SAM)~\cite{foret_sharpness-aware_2021,andriushchenko_sharpness-aware_2023}, will also have small Gaussian width of the featurizer. 

%\yzcomment{After reading the results, I think the values of $\tilde \beta$ and $\beta$ really matter for the bound to be small, i.e.,$O(\sqrt{\log p})$. We can control $\tilde \beta$ by setting a large $m$. But we may need to justify that $\rho$ is not large (by experiment?) so that $\beta$ is smaller than 1 with high probability. Basically, this is saying that if the weights did not move too far away from initialization, then the bound is small. }
%\abcomment{The result needs more thought. Its an upper bound, so we are not saying $\tilde{\beta} < 1$ is necessary. Also need to check the condition on $L$.}
% \begin{remark}
% \abcomment{update as needed}
% Note that choosing $\sigma_1 < 1 - \frac{\rho}{\sqrt{m}}$, which leads to mildly smaller initialization variance, satisfies $\beta < 1$. In this setting, having more depth $L$, at least $\Omega(\log m)$ helps in keeping the Guassian width small. Further, for $\beta=1$, we have $w(\Gamma_{\ffn}) = O(\sqrt{m} \log p)$ which is considerably better than the default $\sqrt{p} = \Theta(\sqrt{L} m)$. Interestingly, for these scenarios, for a suitably large but fixed $p$, having more depth $L$ and less width $m$ helps to keep the Gaussian width upper bound small. \qed 
% \end{remark}


